On Non-Interactive Simulation of Distributed Sources with Finite Alphabets

This work presents a Fourier analysis framework for the non-interactive source simulation (NISS) problem. Two distributed agents observe a pair of sequences $X^d$ and $Y^d$ drawn according to a joint distribution $P_{X^dY^d}$. The agents aim to generate outputs $U=f_d(X^d)$ and $V=g_d(Y^d)$ with a joint distribution sufficiently close in total variation to a target distribution $Q_{UV}$. Existing works have shown that the NISS problem with finite-alphabet outputs is decidable. For the binary-output NISS, an upper-bound to the input complexity was derived which is $O(\exp\operatorname{poly}(\frac{1}{\epsilon}))$. In this work, the input complexity and algorithm design are addressed in several classes of NISS scenarios. For binary-output NISS scenarios with doubly-symmetric binary inputs, it is shown that the input complexity is $\Theta(\log{\frac{1}{\epsilon}})$, thus providing a super-exponential improvement in input complexity. An explicit characterization of the simulating pair of functions is provided. For general finite-input scenarios, a constructive algorithm is introduced that explicitly finds the simulating functions $(f_d(X^d),g_d(Y^d))$. The approach relies on a novel Fourier analysis framework. Various numerical simulations of NISS scenarios with IID inputs are provided. Furthermore, to illustrate the general applicability of the Fourier framework, several examples with non-IID inputs, including entanglement-assisted NISS and NISS with Markovian inputs are provided.

==> NotationHeader.tex <==
%===============================================================================
%------------------------- Special Notations -----------------------------------
%===============================================================================
%++++++++++++++++++++++++   NISS Symbols ++++++++++++++++++++++++++++++++++++
\def\QNISS{\mathcal{Q}(P_{XY}, \mathcal{U}, \mathcal{V})}
\def\Qpartition{\mathcal{P}(P_{X,Y},Q_U,Q_V)}
\def\FBoolQUV{\mathcal{F}_{X Y}}
\def\ENISS{\mathcal{E}(P_{X,Y},Q_U,Q_V)}


%++++++++++++++++++++++++   Fourier Symbols ++++++++++++++++++++++++++++++++++++
\def\fSu{\mathtt{f}_{\mathcal{S}}}
\def\fS{{f}_{\mathcal{S}}}

\newcommand\fSset[1]{{f}_{#1} }
\newcommand\gSset[1]{{g}_{#1} }







\def\fSi{\mathtt{f}_{\mathcal{S}_i}}
\def\fSj{\mathtt{f}_{\mathcal{S}_j}}

\def\ftS{{f}_{\mathcal{S}}}
\def\ftSi{{f}_{\mathcal{S}_i}}
\def\ftSj{{f}_{\mathcal{S}_j}}

\def\fJ{{\mathtt{f}}^{\subseteq \mathcal{J}}}
\def\ftJ{{f}^{\subseteq \mathcal{J}}}
\newcommand\ftsubset[1]{{f}^{\subseteq #1}}


\def\ftJstar{{f}^{\subseteq {\mathcal{J}^*}}}
\def\hJ{h_{\mathcal{J}}}

\def\gSu{\mathtt{g}_{\mathcal{S}}}
\def\gS{{g}_{\mathcal{S}}}
\def\gtS{{g}_{\mathcal{S}}}

\def\gJ{g^{\subseteq J}}

\def\ps{\phi_\mathcal{S}}
\def\pS{\ps}
\def\pSi{\phi_{\mathcal{S}_i}}
\def\pSj{\phi_{\mathcal{S}_j}}
\newcommand{\pset}[1]{{\phi}_{#1}}

\def\ptS{{\psi}_\mathcal{S}}
\def\ptSi{{\psi}_{\mathcal{S}_i}}
\def\ptSj{{\psi}_{\mathcal{S}_j}}
\newcommand{\ptset}[1]{{\psi}_{#1}}

\def\ptildS{\tilde{\psi}_\mathcal{S}}
\def\ptildSi{\tilde{\psi}_{\mathcal{S}_i}}
\def\ptildSj{\tilde{\psi}_{\mathcal{S}_j}}
\newcommand{\ptildset}[1]{\tilde{\psi}_{#1}}





%++++++++++++++++++++++++   Esimation Symbls ++++++++++++++++++++++++++++++++++++
\def\festS{\hat{\mathtt{f}}_{ S} }
\def\festSi{\hat{\mathtt{f}}_{\mathcal{S}_i}}
\def\festSj{\hat{\mathtt{f}}_{\mathcal{S}_j}}



\def\festJ{\hat{\mathtt{f}}^{\subseteq \mathcal{J}}}
\def\festtJ{\hat{{f}}^{\subseteq \mathcal{J}}}


\def\fbarS{\bar{f}_{ S} }
\def\fbarJ{\bar{f}^{\subseteq \mathcal{J}}}


\def\festtS{\hat{f}_{\mathcal{S}}}
\def\festtSi{\hat{f}_{\mathcal{S}_i}}
\def\festtSj{\hat{f}_{\mathcal{S}_j}}




%\def\FestS{\hat{\mathsf{F}}_{S} }
\def\FestS{\festS}

%\def\FestJ{\hat{\mathsf{F}}^{\subseteq \mathcal{J}}}
\def\FestJ{\festJ}

\def\FestSone{\hat{f}_{(1), S} }
\def\FestJone{\hat{f}_{(1)}^{\subseteq \mathcal{J}}}
\def\FestJi{\hat{f}_{(i)}^{\subseteq \mathcal{J}}}
\def\FJibar{\bar{f}_{(i)}^{\subseteq \mathcal{J}}}
\def\FJonebar{\bar{f}_{(1)}^{\subseteq \mathcal{J}}}
\def\FSonebar{\bar{f}_{(1), S} }

\def\pestS{\widehat{\phi}_{\mathcal{S}}}
\def\pesttS{\widehat{\psi}_\mathcal{S}}
\newcommand\pestsubset[1]{\widehat{\psi}_{#1}}
\def\PestS{\widehat{\Psi}_{\mathcal{S}}}

\def\fJbar{f^{\subseteq \bar{J}}}



%++++++++++++++++++++++++   Algorithm Symbls ++++++++++++++++++++++++++++++++++++

\def\Jalg{\hat{\mathcal{J}}_n}
\def\falg{\hat{f}^{\subseteq \Jalg}}
\def\fJalg{{f}^{\subseteq \Jalg}}

\def\predict{\hat{g}}
\def\Peg{P_e(\predict)}


\def\Jalgb{\hat{\mathcal{J}}_2}
\def\falgb{\hat{f}^{\subseteq \Jalgb}}
\def\fJalgb{{f}^{\subseteq \Jalgb}}
\def\predictb{\hat{g}_2}





\def\rndJalg{\mathscr{J}_{alg1}}
\def\rndfalg{\mathsf{F}_{est}^{\subseteq \rndJalg}}
\def\rndpredict{\mathsf{G}_{alg1}}
\def\frndJalg{{f}^{\subseteq \rndJalg}}
\def\L2{\mathcal{L}^2(\mathcal{X}, P_{X^d})}
\def\Pspace{(\mathcal{X},P_{X^d})}





\newcommand{\Pek}{P_{opt}(k)}

\def\mone{M_n}
\def\monebar{\overline{M}_n}
\def\score{\mone}
\def\imscore{\mone}


\def\mtwo{M_n^{(2)}}

\def\E_mu{\mathcal{E}_{\mu}(\epsilon')}
\def\empD{\hat{D}_n}
\def\empLoss{L_{\empD}}
\def\Loss{L_D}
\def\optempLoss{L^*_{\empD}}
\def\optLoss{L^*_D}
\def\empftJ{\festtJ}


\def\Piest{\hat{\Pi}_Y}
\def\Piy{\Pi_Y}
\def\Pibar{\bar{\Pi}_Y}
\def\PiJ{\Pi_Y^{\mathcal{J}}}




\DeclareRobustCommand{\rchi}{{\mathpalette\irchi\relax}}
\newcommand{\irchi}[2]{\raisebox{\depth}{$#1\chi$}} % inner command, used by \rchi

==> PackageHeader2023.tex <==
%=============================================================================
%------------------  Basic Packages -----------------------------------------
%=============================================================================

\usepackage{amsmath}
\usepackage{amsfonts}
%\usepackage{amsthm}   % not compatible with JMLR class
\usepackage{mathrsfs}
\usepackage{tikz}
%\usepackage{mathdots}
\usepackage[utf8]{inputenc}
%\usepackage[ margin=1in ]{geometry}

\usepackage{epstopdf}
\usepackage{mathtools}
\usepackage{graphicx}
%\usepackage{relsize}
%\usepackage{xy}
%\input{xypic}
\usepackage{bbm}
%\setlength{\footskip}{20pt}
\usepackage{enumerate}
\usepackage{epsf,verbatim,amssymb,cite,array,multicol,multirow}  
\usepackage{psfrag,bm,xspace}
%\usepackage{slashbox}
\usepackage{hhline}
%\usepackage{mathabx} % Not stable and incompatible with physics
\usepackage{xstring}
\usepackage{ifthen}
%\pagestyle{plain}
%\usepackage{breakcites} %!! Not compatible with \cite.
\usepackage{booktabs} 



%\def\old@comma{,}
%\catcode`\,=13
%\def,{%
%  \ifmmode%
%    \old@comma\discretionary{}{}{}%
%  \else%
%    \old@comma%
%  \fi%
%}
%\makeatother

%=============================================================================
%---------------------------  Quantum Packages  ------------------------------
%=============================================================================
\usepackage{xparse}
\usepackage{physics}

%=============================================================================
%---------------------------  Algorithms Packages  ------------------------------
%=============================================================================

%\usepackage{algorithm}      % algorithm
%\usepackage[noend]{algpseudocode} % algorithm
%\usepackage[linesnumbered,ruled,vlined,procnumbered]{algorithm2e}

%=============================================================================
%------------------  Basic Theorem Enviroments -----------------------------------------
%=============================================================================

%\newtheorem{thm}{Theorem}
\ifdefined \theorem 
\else
  \newtheorem{theorem}{Theorem}
\fi
%%
%

\ifdefined \lemma 
\else
  \newtheorem{lemma}{Lemma}
  \newtheorem{lem}{Lemma}
\fi

% \newtheorem{lem}{Lemma}
% \newtheorem{lemma}{Lemma}
%
%%\newtheorem{corollary}{Corollary}
%\newtheorem{cor}{Corollary}
%
\ifdefined \corollary 
\else
\newtheorem{corollary}{Corollary}
\fi


\newtheorem{fact}{Fact}

\ifdefined \proposition 
\else
\newtheorem{proposition}{Proposition}
\fi


%\newtheorem{claim}{Claim}
%
\ifdefined \definition 
\else
%\theoremstyle{definition}
\newtheorem{definition}{Definition}
\fi

\ifdefined \example 
\else
\newtheorem{example}{Example}
\fi


\ifdefined \remark 
\else
%\theoremstyle{remark}
\newtheorem{remark}{Remark}
\fi

\ifdefined \conjecture 
\else
\newtheorem{conjecture}{Conjecture}
\fi

\newtheorem{innercustomgeneric}{\customgenericname}
\providecommand{\customgenericname}{}
\newcommand{\newcustomtheorem}[2]{%
  \newenvironment{#1}[1]
  {%
   \renewcommand\customgenericname{#2}%
   \renewcommand\theinnercustomgeneric{##1}%
   \innercustomgeneric
  }
  {\endinnercustomgeneric}
}

\newcustomtheorem{customthm}{Theorem}
\newcustomtheorem{customlemma}{Lemma}
  
  

%-----------------------------------------------------------------------------------------

% makes automatic splits of equations and commas
%%\allowdisplaybreaks 
\makeatletter
\def\old@comma{,}
\catcode`\,=13
\def,{%
  \ifmmode%
    \old@comma\discretionary{}{}{}%
  \else%
    \old@comma%
  \fi%
}
\makeatother

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

%=============================================================================
%------------------  Tracking the changes  -----------------------------------
%=============================================================================
\usepackage{xcolor}
\definecolor{darkblue}{rgb}{0.1,0.1,0.8}
\definecolor{DarkGreen}{rgb}{0,0.6,0}
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\definecolor{britishracinggreen}{rgb}{0.0, 0.26, 0.15}
\definecolor{calpolypomonagreen}{rgb}{0.12, 0.3, 0.17}
\definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
	\definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}
\definecolor{burgundy}{rgb}{0.5, 0.0, 0.13}
\usepackage{etoolbox}

\providetoggle{Blue_revision}
\settoggle{Blue_revision}{true}
\newcommand{\revcol}{\iftoggle{Blue_revision}{\color{blue}}{ }}
\newcommand{\add}[1]{\iftoggle{Blue_revision}{{\color{darkblue}#1}}{ }}
\newcommand{\change}[2]{\iftoggle{Blue_revision}{{\footnotesize \color{brickred}#1}{\color{darkblue}#2}}{ }}

%================  Tracking Multiple Versions ==================================
\providetoggle{Track}
\settoggle{Track}{true}
\newcommand{\addv}[3]{%
	\iftoggle{Track}{%
    	\IfEqCase{#1}{%
       	 	{a}{\ifthenelse{\equal{#2}{ON}}{{\color{cadmiumgreen}#3}}{#3}}%
        	{b}{\ifthenelse{\equal{#2}{ON}}{{\color{brickred}#3}}{#3}}%
       		{c}{\ifthenelse{\equal{#2}{ON}}{{\color{burgundy}#3}}{#3}}%
        	% you can add more cases here as desired
    	}[\PackageError{tree}{Undefined option to tree: #1}{}]%
	}{#3}%
}

%\newcommand{\add}[3]{\iftoggle{#1}{{\color{#2}#3}}{ }}
%\newcommand{\change}[4]{\iftoggle{#1}{{\footnotesize \color{#2}#3}{\color{darkblue}#4}}{ }}



%================  Hyper Cross References ==================================

 \usepackage{hyperref}
%\usepackage{xcolor}


\hypersetup{
colorlinks=true, %
  pdfstartview={FitH},
    linkcolor=red,
    citecolor=blue,
    urlcolor={blue!80!black}
}


\usepackage{graphicx}

%=============================================================================
%---------  Automatic Labeling equality and inequalities  --------------------
%=============================================================================


\newcounter{relctr} %% <- counter for relations
\everydisplay\expandafter{\the\everydisplay\setcounter{relctr}{0}} %% <- reset every eq
\renewcommand*\therelctr{\alph{relctr}} %% <- label format

\newcommand\mystackrel[2]{%
  \begingroup
    \refstepcounter{relctr}%
    \stackrel{\text{(\alph{relctr})}}{\mathstrut{#1}}%
    \originallabel{#2}%
  \endgroup
}
\AtBeginDocument{\let\originallabel\label} %% <- store original definition

\newcommand{\etal}{\textit{et al. }}


%========================================================================================
%------------------------- Shorthands and General Notations -----------------------------
%========================================================================================
\newcommand{\prodin}{\prod_{i=1}^n}
\newcommand{\sumin}{\sum_{i=1}^n}

%====================== double script fonts  =====================================

\global\long\def\RR{\mathbb{R}}
\global\long\def\CC{\mathbb{C}}
\global\long\def\NN{\mathbb{N}}
\global\long\def\QQ{\mathbb{Q}}
\global\long\def\ZZ{\mathbb{Z}}
\global\long\def\EE{\mathbb{E}}
\global\long\def\PP{\mathbb{P}}
\global\long\def\FF{\mathbb{F}}
\global\long\def\11{\mathbbm{1}}

%====================== math bold fonts  =====================================
\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}

\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}

\newcommand{\clA}{\mathcal{A}}
\newcommand{\clB}{\mathcal{B}}
\newcommand{\clC}{\mathcal{C}}
\newcommand{\CJ}{\mathcal{J}}
\newcommand{\clH}{\mathcal{H}}
\newcommand{\ClM}{\mathcal{M}}
\newcommand{\CP}{\mathcal{P}}
\newcommand{\CS}{\mathcal{S}}
\newcommand{\CT}{\mathcal{T}}
\newcommand{\CU}{\mathcal{U}}
\newcommand{\CV}{\mathcal{V}}
\newcommand{\CX}{\mathcal{X}}
\newcommand{\CY}{\mathcal{Y}}
\newcommand{\clY}{\mathcal{Y}}


%====================== shortcuts for operators  =====================================

\global\long\def\+{\oplus}
\global\long\def\P{\mathsf{P}}
\global\long\def\dd{\cdots}
\newcommand\pmm{\{-1,1\}}

\newcommand{\prob}[1]{\PP\Big( #1 \Big) }
\def\<{\langle}
\def\>{\rangle}

%\newcommand{\sign}{\mathsf{sign}}
\DeclareMathOperator*{\sign}{sign}



\ifdefined \var 
  \renewcommand{\var}{\mathsf{var}}
\else
  \newcommand{\var}{\mathsf{var}}
\fi

\ifdefined \abs \else
 \newcommand{\abs}[1]{\lvert#1\rvert}
\fi

\ifdefined \norm \else
 \newcommand{\norm}[1]{\lVert#1\rVert}
\fi


\ifdefined \set 
  \renewcommand{\set}[1]{\left\{#1\right\}}
\else
  \newcommand{\set}[1]{\left\{#1\right\}}
\fi


\DeclareMathOperator*{\supp}{supp}

\newcommand*{\medcap}{\mathbin{\scalebox{1}{\ensuremath{\bigcap}}}}%
\newcommand*{\medcup}{\mathbin{\scalebox{1}{\ensuremath{\bigcup}}}}%
\newcommand*{\medprod}{\mathbin{\scalebox{1}{\ensuremath{\prod}}}}%

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

%-------- delta = for definition -----
\usepackage{stackengine}
\def\deq{\mathrel{\ensurestackMath{\stackon[1pt]{=}{\scriptstyle\Delta}}}}

